Weakly Supervised Open-Vocabulary Object Detection

Despite weakly supervised object detection (WSOD) being a promising step toward evading strong instance-level annotations, its capability is confined to closed-set categories within a single training dataset. In this paper, we propose a novel weakly supervised open-vocabulary object detection framework, namely WSOVOD, to extend traditional WSOD to detect novel concepts and utilize diverse datasets with only image-level annotations. To achieve this, we explore three vital strategies, including dataset-level feature adaptation, image-level salient object localization, and region-level vision-language alignment. First, we perform data-aware feature extraction to produce an input-conditional coefficient, which is leveraged into dataset attribute prototypes to identify dataset bias and help achieve cross-dataset generalization. Second, a customized location-oriented weakly supervised region proposal network is proposed to utilize high-level semantic layouts from the category-agnostic segment anything model to distinguish object boundaries. Lastly, we introduce a proposal-concept synchronized multiple-instance network, i.e., object mining and refinement with visual-semantic alignment, to discover objects matched to the text embeddings of concepts. Extensive experiments on Pascal VOC and MS COCO demonstrate that the proposed WSOVOD achieves new state-of-the-art compared with previous WSOD methods in both close-set object localization and detection tasks. Meanwhile, WSOVOD enables cross-dataset and open-vocabulary learning to achieve on-par or even better performance than well-established fully-supervised open-vocabulary object detection (FSOVOD).

==> Tables/table_ablation_recall_coco.tex <==
\begin{table}[t]
    \caption{
        Compared with learning-free and learning-based methods on all $80$ COCO classes average recall~(AR) on average IoU$_{0.5:1.0}$.
    }
    \begin{center}
        \begin{adjustbox}{max width=0.49\textwidth}
            \begin{tabular}{l|ccc}
                \toprule
                Method&AR@$10$&AR@$100$&AR@$1,000$\\
                 
                \midrule

                \multicolumn{4}{c}{Learning-free Methods} \\

                \midrule
                
                EdgeBoxes~\cite{zitnick2014edge}&7.4&17.8&33.8\\

                Geodesic~\cite{krahenbuhl2014geodesic}&4.0&18.0&35.9\\

                Sel.Search~\cite{uijlings2013selective}&5.2&16.3&35.7\\

                MCG~\cite{pont2016multiscale}&10.1&24.6&39.8\\

                \midrule
                \multicolumn{4}{c}{Learning-based Methods} \\
                \midrule
                
                DeepMask~\cite{o2015learning}&13.9&28.6&43.1\\

                OLN-Box~\cite{kim2022learning}&$\mathbf{27.7}$&46.1&55.7\\

                \midrule
                
                Ours&16.9&$\mathbf{47.3}$&$\mathbf{57.7}$\\
                
                \bottomrule
            \end{tabular}
        \end{adjustbox}
    \end{center}
    \label{table_ablation_recall_coco}
\end{table}

